Optimal Semantic-aware Sampling and Transmission in Energy Harvesting Systems Through the AoII

We study a real-time tracking problem in an energy harvesting status update system with a Markov source and an imperfect channel, considering both sampling and transmission costs. The problem primary challenge stems from the non-observability of the source due to the sampling cost. By using the age of incorrect information (AoII) as a semantic-aware performance metric, our main goal is to find an optimal policy that minimizes the time average AoII subject to an energy-causality constraint. To this end, a stochastic optimization problem is formulated and solved by modeling it as a partially observable Markov decision process (POMDP). More specifically, to solve the main problem, we use the notion of a belief state and cast the problem as a belief MDP problem. Then, for the perfect channel setup, we effectively truncate the corresponding belief space and solve the MDP problem using the relative value iteration method. For the general setup, a deep reinforcement learning policy is proposed. The simulation results show the efficacy of the derived policies in comparison to an AoI-optimal policy and an opportunistic baseline policy.

==> Chapters/backupfiles.tex <==




++++++++++++++++



\begin{align}
     b_i(t)\triangleq \Pr\{\delta(t) = i\,|\,I^{\mathrm{C}}(t)\}, ~  
\end{align}
The belief update, which is a function of the  current belief ${ b_i(t),\, i\in\{0,1,\dots\} }$ and the current action $a(t)$ 
is given by: 
     \\
If $a(t) = 0$:
  \begin{equation}
     \begin{array}{ll}
 b_i(t+1) =
 \left\{ 
  \begin{array}{ll}
   b_0(t)p + (1-b_0(t))(1-p), & i=0,
   \\
 (1-p)  b_{0}(t)  , & i= 1,
    \\
 p  b_{i-1}(t)  , & i= 2,3,\ldots, 
\end{array}\right. 
    \end{array}
 \end{equation}
 and if $a(t) = 1$:
  \begin{equation}
     \begin{array}{ll}
 b_i(t+1) =
 \left\{ 
  \begin{array}{ll}
  p, & i=0,
   \\
 1-p,   & i= 1,
    \\
0  , & i= 2,3,\ldots. 
\end{array}\right. 
    \end{array}
 \end{equation}
%  \end{Pro}
We can now formulate a  continuous-state
MDP by defining its state as  
% \begin{equation}
%     \begin{array}{cc}
       $ z(t) \triangleq \left( e(t), \{b_i(t)\}_{i= 0,1,\ldots}\right)$,
       and 
       its immediate cost function as
$
 { c(z(t)) = \sum_{i} b_i(t)i,~i\in\{0,1,\dots\}.}
$
%     \end{array}
% \end{equation}
Moreover, let $\mathcal{Z}$ denote the corresponding state space.

% The immediate cost function is defined by
% $
%  { c(z(t)) = \sum_{i} b_i(t)i,~i\in\{1,2,\dots\}.}
% $

Now, the main objective is to find the optimal policy ${ \pi^*: \mathcal{Z}\rightarrow \mathcal{A} }$ that is a solution of the following problem:
\begin{equation}\label{Eq_Prob_AoIIMDP}
    \begin{array}{cc}
       %\pi^*({z(0)}) =
       \arg\min_{\pi\in\Pi} ~ 
      \left\{ \limsup_{T\rightarrow \infty}\frac{1}{T}  \sum_{t=1}^T \Bbb{E}\{ c(z(t))\,\big|\,z(0) \}
      \right\},
    \end{array}
\end{equation}
where the expectation is with respect to the policy and the system randomness, and $\Pi$ is the set of all admissible policies.

Although problem \eqref{Eq_Prob_AoIIMDP} is an MDP problem and tools from dynamic programming might be applied to solve it, its state space $\mathcal{Z}$ is a potentially \textit{infinite} set, making it extremely challenging to find an efficient policy.
Nonetheless, we will characterize the state space using the AoI (at the monitor), which allows us  to find an optimal policy. 

Let   ${ \theta(t)\in\{1,2,\dots\} }$ be the AoI, which evolves as 
\begin{equation}\label{Eq_AoITr}
    \begin{array}{cc}
        \theta(t+1) =\left\{ 
  \begin{array}{ll}
      1, & \text{if} ~ a(t) = 1, 
 \\
 \theta(t) + 1, & \text{otherwise}.
    \end{array}
    \right.
    \end{array}
\end{equation}
\indent
Suppose $\theta(t) = n$, $n=1,2,\dots$. Then the belief at each slot $t$ can be written as 
   \begin{equation}\label{Eq_AoII_BD}
     \begin{array}{cc}
 b_i(t) =
\left\{\begin{array}{ll}
  g(n), & i=0,
   \\
g(n-i)(1-p)p^{(i-1)} , & i= 1,\dots,n,
   \\
  0, & i=n+1,\dots,
 \end{array}\right. 
    \end{array}
 \end{equation}
 where the function $g(n)$ is given by
 \begin{equation}\nonumber
     \begin{array}{ll}
        g(n) \triangleq \Pr\{\delta(t) = 0\,|\,\theta(t)=n\}
 =
 0.5(1+(2p-1)^n),
     \end{array}
 \end{equation}
 and $g(0) = 1$. 

 Now, from \eqref{Eq_AoII_BD}, one can observe that,  for sufficiently large values of  the AoI $\theta(t)$, denoted by $N$,   the belief corresponding to $\theta(t)=N$, converges to the following: 
    \begin{equation}\label{}
     \begin{array}{cc}
 b_i(t) =
\left\{\begin{array}{ll}
  0.5, & i=0,
   \\
g(N-i)(1-p)p^{(i-1)} , & i= 1,\dots,N,
   \\
  0, & i=N+1,\dots.
 \end{array}\right. 
    \end{array}
 \end{equation}
 Thus, we can effectively truncate the belief space by bounding the AoI with $N$. We will numerically show the impact of $N$ on the performance of the derived policy (see Fig. \ref{Fig_impactofN}).

\textit{MDP formulation:}
 Now, one interesting conclusion is that both the cost function and belief state at each slot $t$ can be written only as a function of the AoI, which is bounded by $N$.
Thus, problem \eqref{Eq_Prob_AoIIMDP} can be re-expressed, only based on the AoI, as a finite-state MDP problem with the following elements:
 % Thus, we have a finite-state MDP for which 
 % the  algorithm is applied to obtain an optimal policy if it convergence.
 \\
$\bullet$
\textit{State:}
The state at slot $t$ is $\underline{s}(t)= \left( e(t), \theta(t)\right),$ where $\theta(t)\in\{1,2,\dots,N\}$. 
Let  $\underline{\mathcal{S}}$ denote the state space,  which is a finite set.
\\
$\bullet$
\textit{Action:} 
The actions are the same as those of  the POMDP.
%, under that fact that 
 % that $\delta(t)=0$ implies the there is no error. 
\\
$\bullet$
\textit{State Transition Probabilities:} 
The (state)  transition probabilities from the current state ${\underline{s} =(e,\theta)}$ to the next state ${\underline{s}'=(e',\theta')}$, given an action $a$, is defined by  
$
{
 \mathcal{P}_{\underline{s}\underline{s}'}(a) =
        \Pr\{\underline{s}'\,|\,\underline{s}, a\} }, 
  $  
which can be written as $ {\Pr\{\theta'\,|\,\theta,\,a\}\Pr\{e'\,|\,e,\theta,a\} } $, where $\Pr\{\theta'\,|\,\theta,a\}$ and $\Pr\{e'\,|\,e,\theta,a\}$, are respectively, given by 
\begin{equation}\label{Eq_AoIDyn}
     \begin{array}{cc}
        \Pr\{\theta'\,|\,\theta,\,a\} =\left\{ 
  \begin{array}{ll}
  1,   & \text{if} ~ a = 0,~ \theta' = \min\{ \theta+1, N\},
  \\
     1,  & \text{if} ~ a = 1,~ \theta'=1,
     \\
     0,  & \text{otherwise}.
    \end{array}
    \right.
     \end{array}
 \end{equation}
\begin{equation}
     \begin{array}{ll}
     &    \Pr\{e'\,|\,e,\theta,\,a\}  =
        \\&
        \left\{ 
  \begin{array}{ll}
  \mu,   & \text{if} ~ a = 0,~ e' = \min\{e+1, E\},
  \\
    1-\mu,   & \text{if} ~ a = 0,~ e' = e,
  \\
  \mu(1-g(\theta)),   & \text{if} ~ a = 1,~ e' = e+1-(c^{\mathrm{s}} + c^{\mathrm{t}}),
  \\
  (1-\mu)(1-g(\theta)),   & \text{if} ~ a = 1,~ e' = e-(c^{\mathrm{s}} + c^{\mathrm{t}}),
    \\
  \mu g(\theta),   & \text{if} ~ a = 1,~ e' = e+1-c^{\mathrm{s}},
  \\
(1-\mu)g(\theta),   & \text{if} ~ a = 1,~ e' = e-c^{\mathrm{s}},
  \\
     0,  & \text{otherwise},
    \end{array}
    \right.
     \end{array}
 \end{equation}
 where $g(\theta) = 0.5(1+(2p-1)^\theta)$.
 \\
 $\bullet$
 \textit{Cost function:}
 The immediate cost function at slot $t$ is the expected AoII and is given by
 \begin{equation}
     C(\underline{s}(t)) = \sum_{i=0}^{\theta(t)} b_i(t)i,~\theta(t)\in\{1,2,\dots,N\}, 
 \end{equation}
where $b_i(t)$ is given by
   \begin{equation}\label{}
  % \nonumber
     \begin{array}{cc}
 b_i(t) =
\left\{\begin{array}{ll}
  g(\theta(t)), & i=0,
   \\
g(\theta(t)-i)(1-p)p^{(i-1)} , & i= 1,\dots,\theta(t).
  %  \\
  % 0, & i=\theta+1,\dots,N.
 \end{array}\right. 
    \end{array}
 \end{equation}

Next, we show that the MDP, specified above, is communicating under which the Bellman’s (optimality) equation (see \cite[Eq. 4.47]{bertsekas2007dynamic})  has a solution and the optimal average AoII
is independent of the initial state $z(0)$ \cite[Proposition 4.2.3]{bertsekas2007dynamic}.

\begin{Pro}\label{Prop_ComMDP}
The MDP is  communicating.  % not unichain but
\end{Pro}
\begin{proof}
%The fact that the MDP is not unichain can be  shown via a counterexample. 
To show the MDP is communicating, we should find a stationary randomized policy that induces a recurrent Markov chain, i.e., 
a policy  under which every pair of states
%${\underline{s}=(e,\theta)}$ and ${ \underline{s}'=(e',\theta')}$
in the state space $\underline{\mathcal{S}}$ is accessible from each other. The details of the proof are deferred to the extended version. 
\end{proof}

 Under Proposition \ref{Prop_ComMDP},
we can find an optimal deterministic policy and the optimal average AoII (which are independent of the initial state), by solving the Bellman's equation \cite[Proposition 4.2.6]{bertsekas2007dynamic}. 
We apply the relative value iteration (RVI) algorithm \cite[Section 4.3]{bertsekas2007dynamic}, which returns an optimal deterministic policy if it converges. 
%\footnote{\red{We shall clarify that there is no guarantee of convergence, as the the unichain structure does not exist.}}.
The RVI algorithm transforms the  Bellman's equation into the following iterative process for each state $s\in\underline{\mathcal{S}}$:
\begin{equation}\label{Eq_RVIal}
\nonumber
\begin{array}{ll}
 a^* \leftarrow  % \underset{ a }{\arg\min}
 \arg\min_{a} 
 \left\{C(\underline{s})+\sum_{\underline{s}^{\prime} \in \underline{\mathcal{S}}} \operatorname{Pr}\left(\underline{s}^{\prime} \mid \underline{s}, a\right) V(\underline{s}^{\prime})\right\},
 %~\forall s\in\mathcal{S}, 
\\
%\textstyle
 V(\underline{s}) \leftarrow\left\{C\left(\underline{s}\right)+
 \sum_{\underline{s}^{\prime} \in \underline{\mathcal{S}}}
 %\underset{s^{\prime} \in \mathcal{S}}{\sum}
 \operatorname{Pr}\left(\underline{s}^{\prime} \mid \underline{s}, a^*\right) V({\underline{s}^{\prime}})\right\}-V({\underline{s}_{\mathrm{ref}}}), 
 %\forall s\in\mathcal{S}, 
\end{array}
\end{equation}
where $\underline{s}_{\mathrm{ref}} \in \underline{\mathcal{S}}$ is an arbitrary chosen reference state. Once the iterative process above converges, the algorithm provides an optimal policy $\pi^*$ and the optimal value of the average AoII, which equals to $V({\underline{s}_{\mathrm{ref}}})$.
